Detecting Metadata-Related Bugs in Enterprise Applications

When building enterprise applications (EAs) on Java frameworks (e.g., Spring), developers often configure application components via metadata (i.e., Java annotations and XML files). It is challenging for developers to correctly use metadata, because the usage rules can be complex and existing tools provide limited assistance. When developers misuse metadata, EAs become misconfigured, which defects can trigger erroneous runtime behaviors or introduce security vulnerabilities. To help developers correctly use metadata, this paper presents (1) RSL -- a domain-specific language that domain experts can adopt to prescribe metadata checking rules, and (2) MeCheck -- a tool that takes in RSL rules and EAs to check for rule violations. With RSL, domain experts (e.g., developers of a Java framework) can specify metadata checking rules by defining content consistency among XML files, annotations, and Java code. Given such RSL rules and a program to scan, MeCheck interprets rules as cross-file static analyzers, which analyzers scan Java and/or XML files to gather information and look for consistency violations. For evaluation, we studied the Spring and JUnit documentation to manually define 15 rules, and created 2 datasets with 115 open-source EAs. The first dataset includes 45 EAs, and the ground truth of 45 manually injected bugs. The second dataset includes multiple versions of 70 EAs. We observed that MeCheck identified bugs in the first dataset with 100% precision, 96% recall, and 98% F-score. It reported 156 bugs in the second dataset, 53 of which bugs were already fixed by developers. Our evaluation shows that MeCheck helps ensure the correct usage of metadata.

==> evaluation-subsections/history-commits.tex <==
\subsection{Fixed Bugs in History Commits}\label{ss:eval-history}

Instead of checking every single commit in the projects, we applied a filtering. We crawled commits where the commit message has 1) bug or fix or error, and 2) metadata or xml or annotation in it. We also made sure that the commits involved changes in .java or .xml files.
\todo{there are some earlier cases where these filterings were not applied}

As we mentioned in \ref{ss:eval-effect-mecheck}, we found \totalInteresting real bugs from \totalInterestingEAs projects. After also checking the latest version of those repositories for the \totalInteresting bugs, we found out that 7 of them has never been addressed by the developers. The other 18 bugs have been fixed or addressed by the developers in later commits.

\vspace{0.5em}
\noindent\begin{tabular}{|p{8.1cm}|}
	\hline
	\textbf{Finding 3:} \emph{There are metadata-related bugs in real-world projects. Most of the bugs (18 out of 24) \tool detected in version history have been fixed by the developers in later commits and they are no longer available in the latest versions.}
	\\
	\hline
\end{tabular}
